The current state of affairs in 5G security and the main remaining security challenges

The first release of the 5G protocol specifications, 3rd Generation Partnership Project (3GPP) Release 15, were published in December 2017 and the first 5G protocol security specifications in March 2018. As one of the technology cornerstones for Vehicle-to-Vehicle (V2X), Vehicle-to-Everything (V2E) systems and other critical systems, 5G defines some strict communication goals, such as massive device connectivity, sub-10ms latency and ultra high bit-rate. Likewise, given the firm security requirements of certain critical applications expected to be deployed on this new cellular communications standard, 5G defines important security goals. As such, 5G networks are intended to address known protocol vulnerabilities present in both legacy GSM (Global System for Mobile Communications) networks as well as current LTE (Long Term Evolution) mobile systems. This manuscript presents a summary and analysis of the current state of affairs in 5G protocol security, discussing the main areas that should still be improved further before 5G systems go live. Although the 5G security standard documents were released just a year ago, there is a number of research papers detailing security vulnerabilities, which are summarized in this manuscript as well.

==> include/architecture.tex <==
One of the main goals for 5G wireless networks is massive connectivity, aiming to be the main enabler for the IoT. There is a common catchphrase in the industry about billions or even trillions of connected embedded devices by 2020, and the 5G guidelines and goals also envision wireless connectivity of a similar order of magnitude. This rapid growth of the IoT, which resulted in the number of connected devices topping the world's population in 2013 \cite{m2m_more_than_humans}, is one of the main foreseeable challenges for communication networks, both in terms of capacity and security.

The massive and unsupervised deployment of low computational power embedded devices over mobile wireless networks results in a highly challenging security landscape. Exploits that are difficult to monetize or that generate a large impact, such as blocking the connectivity of mobile endpoints \cite{LTEpracticalattacks}, are substantially more concerning in the context of critical M2M applications\footnote{Known exploits block the connectivity of mobile devices until rebooted or forced a connection reestablishment. Launching such an attack against a large deployment of M2M sensors could result in a lengthy DoS, as it is costly and time consuming to send technicians to manually reboot all the impacted M2M sensors. Security concerns and the stakes are especially high if such deployments belong to either physical security or healthcare systems.}. On top of that, sophisticated authentication and encryption techniques, such as the ones discussed in Section \ref{sec:publickey}, are very challenging to implement in low-power embedded devices. Despite this being one of the main security challenges of 5G (in the context of IoT), there is a lot of excellent work in both industry and academia aimed at tackling these problems. This document aims to highlight the main architectural challenges of 5G mobile networks in the context of the IoT surge -- a challenge that will only be exacerbated if mobile connectivity indeed reaches billions or trillions.

The concept of mobile core overloading due to control plane signaling was first introduced in \cite{lee_dos}, which described a theoretical signaling overload threat against cellular networks. A low-volume attack, consisting of small data packets addressed to a large number of mobile devices, would theoretically induce a large number of RRC state transitions and, theoretically, overload the packet core of a mobile network.

\begin{table}[h]
\begin{center}
    \begin{tabular}{|p{4.5cm}|p{9.2cm}|M|}
    \hline
    \hline
    Cause                       & Event                                                                       & Reference          \\ \hline \hline
    Chatty app                  & IM app checking for new messages too frequently caused outage at U.S. carrier & \cite{TMobile}            \\ \hline
    Signaling spike             & Outage for 3 million users at the world's 6th largest operator & \cite{Telenor}            \\ \hline
    Smartphone native apps      & Native apps from one of the main mobile OSes caused signaling overloads on Japanese mobile network                         & \cite{Docomo}             \\ \hline
    Chatty apps                 & Operators at Open Mobile Summit discuss actions to mitigate signaling spikes from chatty apps & \cite{chattyApps}         \\ \hline
    Adds in popular app         & Signaling spikes caused by ads displayed in a popular mobile game           & \cite{AngryBirds_storm}  \\ \hline
    LTE-connected tablet        & Connectivity from popular tablet substantially increases control plane signaling & \cite{ipad_storm}        \\ \hline
    Mobile cloud service        & Frequent reconnect attempts to a cloud service under outage resulted in signaling spike & \cite{OTTblackout_storm} \\ \hline \hline
    \end{tabular}
\end{center}
\label{tab:signalingstorms}
    \caption{Sample of known signaling overload events \cite{jover2015bookchapter}}
\end{table}

This doomsday scenario, initially conceived as an adversarial threat, started to become a reality in the wild with the advent of the smartphone and mobile app stores. This is when the term \emph{signaling storm}, also referred to as \emph{signaling tsunami} in eye-catching media headlines, was coined. This availability threat against the mobile core infrastructure arises, yet again, from the long overdue need for mobile networks to completely reinvent themselves and take a leap away from legacy technologies. Specifically, the circuit-switched core architecture of mobile systems, nicely suited to carry circuit-switched traffic - phone calls - that fits a Poisson arrival process with exponentially distributed call duration, is not the right architecture to transport the bursty IP-based traffic from billions of modern devices.

The more the Internet traffic from a consumer device differed from a classic Markov process, the more this issue became apparent. A simple Google search for the term \texttt{signaling storm} returns dozens of major outages at large cell operators due to spikes in control plane signaling traffic originated by constantly bringing up and tearing down circuits for the bursty packetized IP traffic from mobile devices. Table \ref{tab:signalingstorms} summarizes a few instances of signaling overloads over the past few years.

As discussed in \cite{lee_dos}, the impact of a malicious spike of control plane traffic could result in a direct threat against the availability of mobile systems. In the current mobile security landscape, it is common to see malicious applications (i.e., malware) infecting tens of thousands of mobile devices, or more, within a short span of time. Often, malware is written with a monetary or fraudulent goal. However, there are concerns across the industry and academia about the potential impact of a botnet of malware-controlled smartphones triggering, for example, a spike of attach procedures by repeatedly toggling airplane mode.

The traffic characteristics of most IoT applications are substantially different from the traffic of smartphones and tablets. It has been known for years that IoT traffic is a potential source for large mobile resource utilization inefficiencies \cite{m2m_pang}. Given that signaling overloads are already impacting the availability of mobile systems, the challenge is obvious – especially when one mixes in an even more heterogeneous mix of billions of devices with bursty traffic flows or, even worst, periodic small flows of data \cite{M2MscalabilityJermyn}.

The current evolution of LTE mobile systems has been addressing the signaling overload problem for years \cite{LTE_SIGNALING_OVERLOADS}. Moreover, the push towards virtualization and Software Defined Networks (SDNs) provides more enhanced scalability for mobile networks. Upon a spike of signaling traffic, the mobile core elements can flexibly have their computing resources expanded to handle the increased control plane load.

Despite these aforementioned technology enhancements to improve mobile connectivity for massive IoT deployments, the architecture of mobile communication systems must be fully redesigned. It has been argued for years that, in the long run, 5G wireless systems must move away from the rigid and non-scalable legacy circuit-switched architecture and aim for a fully packet-switched infrastructure, not too different from today's IP networks \cite{kim2012directions}. 

==> include/related.tex <==
The wide availability of open source tools for GSM experimentation has fueled a large array of very interesting security research on legacy networks. From the first demonstrations of GSM traffic interception and eavesdropping \cite{attack_sniffing} to DoS threats against the GSM air interface \cite{attack_RACH_GSM1}, a number of GSM exploits have been reported in the literature and security conferences. Privacy and location leaks have also been deeply investigated in the context of legacy GSM networks \cite{kune2012location}.

LTE security research has been increasingly predominant over the last couple of years, mainly in network availability related projects. For example, there has been interesting studies aiming to quantify and investigate the impact of large spikes of traffic load originated from M2M systems against the LTE infrastructure \cite{m2m_phy_impact_modeling}. Also in the context of M2M, several studies have focused on the control plane signaling impact of the IoT against the LTE mobile core \cite{jaber2014cellular,M2MscalabilityJermyn}.

Applied LTE security research and protocol exploit experimentation have been close to non-existent over the last few years. However, the recent availability of open source tools for LTE experimentation have provided the means for very interesting security research work. For example, some recent studies aimed at analyzing and evaluating sophisticated jamming threats against LTE networks \cite{lichtman2013security,lichtman2013vulnerability}. Also leveraging LTE open source tools, the authors of \cite{LTEpracticalattacks} were the first to publicly disclose the implementation and analysis of the device blocking and soft downgrade to GSM exploits, which were also implemented in this manuscript. The same authors are responsible for some other excellent mobile protocol exploit experimentation, such as a study on intercepting phone calls and text messages in GSM networks \cite{golde2013letmeanswer} and mobile phone baseband fuzzing \cite{mulliner2011smsfuzzing}. 
